A Core Calculus for Provenance

Provenance is an increasing concern due to the ongoing revolution in sharing and processing scientific data on the Web and in other computer systems. It is proposed that many computer systems will need to become provenance-aware in order to provide satisfactory accountability, reproducibility, and trust for scientific or other high-value data. To date, there is not a consensus concerning appropriate formal models or security properties for provenance. In previous work, we introduced a formal framework for provenance security and proposed formal definitions of properties called disclosure and obfuscation. In this article, we study refined notions of positive and negative disclosure and obfuscation in a concrete setting, that of a general-purpose programing language. Previous models of provenance have focused on special-purpose languages such as workflows and database queries. We consider a higher-order, functional language with sums, products, and recursive types and functions, and equip it with a tracing semantics in which traces themselves can be replayed as computations. We present an annotation-propagation framework that supports many provenance views over traces, including standard forms of provenance studied previously. We investigate some relationships among provenance views and develop some partial solutions to the disclosure and obfuscation problems, including correct algorithms for disclosure and positive obfuscation based on trace slicing.

==> fig-approach.tex <==
\begin{figure}
\centering
%
\parbox{0.90\columnwidth}{
\xymatrixcolsep{3pc}
\xymatrixrowsep{2.5pc}
\xymatrix{
X\ar[r]^a_b & Y & Z\ar[l]^A_B 
\\
e
\ar@{->}[r]
&
T
\\
}
}%% e'
%% %\ar@{=}[d]
%% \ar[r]^{top2}_{bottom2}
%% &
%% S\ar@{=}[d]|{\mbox{\small down3}}
%% \s^\tgtX; T_0^\tgtX \ar[r]^{\curvearrowright^\tgtX} 
%% & 
%% v'
%
%% \hfill
%% %
%% \parbox{0.5\columnwidth}{
%% \xymatrixcolsep{5pc}
%% \xymatrixrowsep{2.5pc}
%% \xymatrix{
%% T_1^\srcX
%% \ar@{.>}[d]|{\mbox{\small translation}}
%% \ar@{<-->}[r]^{\trdCP^\srcX}_{d^\srcX}
%% &
%% T_2^\srcX \ar@{.>}[d]|{\mbox{\small translation}}
%% \\
%% T_1^\tgtX
%% \ar@{=}[d]
%% %% \ar@{<-->}[r]^{\Delta^\tgtX = O(d^\srcX)}_{\Delta^\tgtX = d^\tgtX}
%% \ar@{<-->}[r]^{\trdCP^\tgtX}_{d^\tgtX \in O(d^\srcX)}
%% &
%% T_2^\tgtX \ar@{=}[d]\\
%% T_1^\tgtX \ar@{<-->}[r]^{\curvearrowright^\tgtX}_{d^\tgtX} & T_2^\tgtX}
%% }
%
\caption{The left diagram illustrates the correspondence between the
  source and target from-scratch runs and the consistency of change
  propagation in the target.  The right diagram illustrates the
  correspondence between distance in the source and target, and the time
  for change propagation in the target.}
\label{fig:approach}
\vspace*{-3mm}
\end{figure}


==> fig-eqpat.tex <==
\begin{figure}[tb]
\fbox{$v \eqpat{p} v$}
\vspace{-3mm}
\begin{smathpar}
\inferrule*{
\strut
}
{v \eqpat{\vhole} v'}
\and
\inferrule*
{
\strut
}
{
v \eqpat{\vany} v
}
\and
\inferrule*
{
\strut
}
{
\vc \eqpat{\vc} \vc
}
\and
\inferrule*
{
\vc \neq \vc_0 \neq \vc'
}
{
\vc \eqpat{\vc_0} \vc'
}
\and
\inferrule*
{
  v_1 \eqpat{p_1} v_1'
  \\
  v_2 \eqpat{p_2} v_2'
}
{
  \vpair{v_1}{v_2} \eqpat{(p_1,p_2)} \vpair{v_1'}{v_2'}
}
\and
\inferrule*{v \eqpat{p} v'}
{\vinl{v} \eqpat{\vinl{p}} \vinl{v'}}
\and
\inferrule*{v \eqpat{p} v'}
{\vinr{v} \eqpat{\vinr{p}} \vinr{v'}}
\and
\inferrule*{v \eqpat{p} v'}
{\vroll{v} \eqpat{\vroll{p}} \vroll{v'}}
\and
\inferrule*{C \neq C_0 \neq C' \\
C,C',C_0 \in \{\kw{inl}, \kw{inr}, \kw{roll}\}}
{C(v) \eqpat{C_0(p)} C'(v')}
%
\and
%
\inferrule*{
\gamma \eqpat{\rho}\gamma'
}
{
\vclos{\kappa}{\gamma} \eqpat{\vclos{\kappa}{\rho}} \vclos{\kappa}{\gamma'}
}
\and
\inferrule*{
\kappa \neq \kappa_0 \neq \kappa'
}
{
\vclos{\kappa}{\gamma} \eqpat{\vclos{\kappa_0}{\rho}} \vclos{\kappa'}{\gamma'}
}
\end{smathpar}
\begin{eqnarray*}
  \gamma \eqpat{\rho} \gamma' &\iff &\forall x \in
  \dom(\rho). ~\gamma(x) \eqpat{\rho(x)} \gamma'(x)
\end{eqnarray*}
\caption{Pattern equivalence of values.}
\label{fig:eqpat}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-example-map-src.tex <==
\begin{figure}
{\small
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`^=7}]
data intlist = Nil | Cons int * intlist

fun map (f: int -> int) (xs : intlist) : intlist =
   case xs of 
      Nil -> Nil
      Cons y -> Cons (f (fst y), map f (snd y))
\end{Verbatim}
}

\vspace{-8pt}
\caption{The code for list map.}
\label{fig:example-map-src}
\end{figure}


==> fig-example-map-traces.tex <==
\begin{figure*}
\begin{minipage}[t]{0.33\textwidth}
\centering
(a) Unsliced trace
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
(b) Slice of \ttt{[\vhole,\vany,\vhole]}
%$
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
(c) Differential slice of  \ttt{[\vhole,\colorbox{Gray}{\vany},\vhole]}
%$
\end{minipage}
\\
\begin{minipage}[t]{0.33\textwidth}
\vspace*{0cm}  % hack to make things align
\includegraphics[scale=0.33]{map-trace-annotated}
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
% Dunno why, but we need to shift some of the pictures up:
% umut: i think tex does not know where the image starts
%\vspace{-3.9in}
\vspace*{0cm}  % hack to make things align
\includegraphics[scale=0.33]{map-slice-annotated}
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
%\vspace{-3.9in}
\vspace*{0cm}  % hack to make thing align
\includegraphics[scale=0.33]{map-slice-diff}
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
\centering{\small Program slice: \ttt{map f [6,7,2]}}
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
\centering {\small Program slice: \ttt{map f [\vhole,7,\vhole]}}
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
\centering
{Program slice: \ttt{map \colorbox{Gray}{f} [\vhole,\colorbox{Gray}{7},\vhole]}}
%$
\end{minipage}

\smallskip

\caption{Trace, slice and differential slice, plus corresponding program slices.}
\label{fig:example-map}
\label{fig:example-map-traces}
\end{figure*}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-example-merge-1.tex <==
\begin{figure}
{\small
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`^=7}]
data intlist = Nil | Cons int * intlist

let merge = fun merge (xs : intlist) (ys : intlist) : intlist =>
  case xs of
    Nil -> ys;
    Cons x -> case ys of 
      Nil -> xs;
      Cons y -> 
        if ((fst x) < (fst y)) 
        then Cons(fst x, merge (snd x) ys)
	else Cons(fst y, merge xs (snd y))
in
   merge 
      (Cons (6, Cons (16, Cons (20, Nil)))) 
      (Cons (3, Cons (12, Cons (13, Nil))))
\end{Verbatim}
%$
}
%\hrule
\caption{Merging two sorted lists.}
\label{fig:example-merge-1}
\end{figure}


==> fig-example-merge-2.tex <==
\begin{figure*}
Slice with respect to 
{\small
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`^=7}]
Cons (\textcolor{Gray}{{$\square$}}, Cons (\textcolor{Gray}{{$\square$}}, Cons (\textcolor{Gray}{{$\square$}}, Cons (13, \textcolor{Gray}{{$\square$}}))))
\end{Verbatim}
}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`^=7}]
let \ul{merge}
  = fun \ul{merge} (\ul{xs}) (\ul{ys}) =>
      case xs of
        Nil -> \textcolor{Gray}{{$\square$}}
        Cons \ul{x} ->
          case ys of
            Nil -> \textcolor{Gray}{{$\square$}}
            Cons \ul{y} ->
              if (fst x) < (fst y)
              then Cons (\textcolor{Gray}{{$\square$}}, merge (snd x) ys)
              else Cons (fst y, merge xs (snd y)) in
\textcolor{RoyalBlue}{merge}
  \ul{xs} = Cons (6, Cons (16, \textcolor{Gray}{{$\square$}}))
  \ul{ys} = Cons (3, Cons (12, Cons (13, \textcolor{Gray}{{$\square$}})))
=> case xs of \textcolor{Mulberry}{Cons} \ul{x} ->
     case ys of \textcolor{Mulberry}{Cons} \ul{y} ->
       if (fst x) < (fst y)
       then Cons (fst x, merge (snd x) ys)
       else Cons
              (\textcolor{Gray}{{$\square$}},
               \textcolor{RoyalBlue}{merge}
                 \ul{xs} = xs
                 \ul{ys} = snd y
               => case xs of \textcolor{Mulberry}{Cons} \ul{x} ->
                    case ys of \textcolor{Mulberry}{Cons} \ul{y} ->
                      if (fst x) < (fst y)
                      then Cons
                             (\textcolor{Gray}{{$\square$}},
                              \textcolor{RoyalBlue}{merge}
                                \ul{xs} = snd x
                                \ul{ys} = ys
                              => case xs of \textcolor{Mulberry}{Cons} \ul{x} ->
                                   case ys of \textcolor{Mulberry}{Cons} \ul{y} ->
                                     if (fst x) < (fst y)
                                     then Cons (fst x, merge (snd x) ys)
                                     else Cons
                                            (\textcolor{Gray}{{$\square$}},
                                             \textcolor{RoyalBlue}{merge}
                                               \ul{xs} = xs
                                               \ul{ys} = snd y
                                             => case xs of \textcolor{Mulberry}{Cons} \ul{x} ->
                                                  case ys of \textcolor{Mulberry}{Cons} \ul{y} ->
                                                    if (fst x) < (fst y)
                                                    then Cons (fst x, merge (snd x) ys)
                                                    else Cons (fst y, \textcolor{Gray}{{$\square$}})))
                      else Cons (fst y, merge xs (snd y)))
\end{Verbatim}
%$
\caption{Trace slice rendered as unrolled expression syntax.}
\label{fig:example-merge-2}
\end{figure*}


==> fig-example-msort-focus-trace.tex <==
\begin{figure}
\centering
\includegraphics[scale=0.43]{sortbug2}
%
\caption{A slice of mergesort with respect to $[\vhole,\vany,\vhole]$;
  the highlighted parts represent the focus on the second element of the list.}
\label{fig:example-msort-focus-trace}

\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-example-msort-src.tex <==
\begin{figure}
{\small
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`^=7}]
data intlist = Nil | Cons int * intlist

fun split (xs : intlist) : intlist * intlist =>
   case xs of 
     Nil -> (Nil,Nil);
     Cons x -> let y = split (snd x) in 
               (Cons(fst x, snd y), fst y)

fun merge (xs : intlist) (ys : intlist) : intlist =>
   case xs of
      Nil -> ys
      Cons x -> case ys of 
                  Nil -> xs
                  Cons y -> 
                     if (fst x) < (fst y)
                        then Cons(fst x,merge (snd x) ys)
                        else Cons(\colorbox{Gray}{fst x},merge xs (snd y))

fun mergesort (xs : intlist) : intlist =>
   case xs of 
      Nil -> Nil;
      Cons x -> case (snd x) of
                   Nil -> Cons(fst x,Nil);
                   Cons y -> let z = split xs in
                                merge (mergesort (fst z)) 
                                      (mergesort (snd z))
\end{Verbatim}
%$
}


%in
%let l = Cons(1,Cons(2,Cons(3,Nil))) in mergesort(l)

\vspace{-8pt}
\caption{The code for buggy mergesort.}
\label{fig:example-msort-src}
\end{figure}


==> fig-example-msort.tex <==
\begin{figure*}
\begin{minipage}{0.47\textwidth}
{\small
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`^=7}]
data intlist = Nil | Cons int * intlist

fun split (xs : intlist) : intlist * intlist =>
   case xs of 
     Nil -> (Nil,Nil);
     Cons x -> let y = split (snd x) in 
               (Cons(fst x, snd y), fst y)

fun merge (xs : intlist) (ys : intlist) : intlist =>
   case xs of
      Nil -> ys
      Cons x -> case ys of 
                  Nil -> xs
                  Cons y -> 
                     if (fst x) < (fst y)
                        then Cons(fst x,merge (snd x) ys)
                        else Cons(\colorbox{Gray}{fst x},merge xs (snd y))

fun mergesort (xs : intlist) : intlist =>
   case xs of 
      Nil -> Nil;
      Cons x -> case (snd x) of
                   Nil -> Cons(fst x,Nil);
                   Cons y -> let z = split xs in
                                merge (mergesort (fst z)) 
                                      (mergesort (snd z))
\end{Verbatim}
%$
}


%in
%let l = Cons(1,Cons(2,Cons(3,Nil))) in mergesort(l)
\vspace{-8pt}
\end{minipage}
%
\hfill
%
\begin{minipage}{0.52\textwidth}
\includegraphics[height=9cm]{sortbug2}
\end{minipage}
\caption{The code for buggy mergesort (left) and a slice of mergesort
  for the focus pattern $[\vhole,\focus{\vany},\vhole]$ isolating the
  second element.}
\label{fig:example-msort}
\end{figure*}


==> fig-example-sort-bug-1.tex <==
\begin{figure*}
   \begin{tabular}[t]{ll}
   (a) & (b)\\
\!\!\!\!\!\!
\includegraphics[scale=0.43]{sortbug1}
&
\!\!\!\!\!\!\!\!\!
\includegraphics[scale=0.43]{sortbug2}
\end{tabular}   
%\hrule
\caption{Say something here.}
\label{fig:example-sort-bug-1}
\end{figure*}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-example-sort-bug-uneval.tex <==
\begin{figure}
{\small
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`^=7}]
fun merge (xs : intlist) (ys : intlist) : intlist =>
   case xs of
      Nil -> ys
      Cons x -> case ys of
                  Nil -> xs
                  Cons y ->
                     if (fst x) < (fst y)
                        then Cons (fst x, merge (snd x) ys)
                        else Cons (\colorbox{Gray}{fst x}, merge xs (snd y))

\end{Verbatim}
%$
}
\vspace{-8pt}
\caption{Differential program slice}
\label{fig:example-sort-bug-uneval}
\end{figure}


==> fig-example-sort-bug.tex <==
\begin{figure}
{\small
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`^=7}]
data intlist = Nil | Cons int * intlist

fun split (xs : intlist) : intlist * intlist =>
   case xs of 
     Nil -> (Nil,Nil);
     Cons x -> let y = split (snd x) in 
               (Cons(fst x, snd y), fst y)

fun merge (xs : intlist) (ys : intlist) : intlist =>
   case xs of
      Nil -> ys
      Cons x -> case ys of 
                  Nil -> xs
                  Cons y -> 
                     if (fst x) < (fst y)
                        then Cons(fst x,merge (snd x) ys)
                        else Cons(\colorbox{Gray}{fst x},merge xs (snd y))

fun mergesort (xs : intlist) : intlist =>
   case xs of 
      Nil -> Nil;
      Cons x -> case (snd x) of
                   Nil -> Cons(fst x,Nil);
                   Cons y -> let z = split xs in
                                merge (mergesort (fst z)) 
                                      (mergesort (snd z))
\end{Verbatim}
%$
}


%in
%let l = Cons(1,Cons(2,Cons(3,Nil))) in mergesort(l)


\vspace{-8pt}
\caption{Buggy mergesort.}
\label{fig:example-copy-list}
\end{figure}


==> fig-example-traces.tex <==
\begin{figure}
   \begin{tabular}[t]{ll}
   (a) & (b)\\
\!\!\!\!\!\!
\includegraphics[scale=0.36]{example}
&
\!\!\!\!\!\!\!\!\!
\includegraphics[scale=0.36]{example-diff}
\end{tabular}   
% \begin{tabular}[t]{ll}
%    (a). & \includegraphics[scale=0.6]{example}
% \\
% (b). &
% \includegraphics[scale=0.6]{example-diff}
% \end{tabular}
%\hrule
\caption{Example trace.  (a) The white nodes form a slice with respect
  to $[\hole,\hole,5,\hole]$. (b) The slice, with differences specific
  to the third element highlighted in gray.  To aid readability, some
  details are omitted.}
\label{fig:example}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-paths.tex <==
\begin{figure}[tb]

  \begin{center}
    \includegraphics[width=2.0in]{lambda-path-example}
  \end{center}

\caption{The paths of $\vpair{\vpair{\vpair{1}{2}}{3}}{\vpair{4}{5}}$.}

\label{fig:paths-example}
\end{figure}

\begin{figure}
\begin{mathfig}
\begin{array}{rcl}

\paths{\kwc} &=& \{\epsilon\}
\\
\paths{(v_1,v_2)} &=& \{1\cdot p \mid p \in \paths{v_1}\}
\\
&\cup & \{2\cdot p \mid p \in \paths{v_2}\}
\\
\paths{\exfun{f}{x}{e}} &=& \{\epsilon\}
\\[2mm]
%

\atpath{v}{\pe} & = & v 
\\
\atpath{\vpair{v_1}{v_2}}{\pcons{1}{p}} & = & \atpath{v_1}{p}
\\
\atpath{\vpair{v_1}{v_2}}{\pcons{2}{p}} & = & \atpath{v_2}{p}
\\[2mm]
%
\mappath{v}{\pe} & = & v
\\
\mappath{\vpair{v_1}{v_2}}{\pcons{1}{p}} & = & \kwpair{\mappath{v_1 }{p}}{\hole}
\\
\mappath{\vpair{v_1}{v_2}}{\pcons{2}{p}} & = & \kwpair{\hole}{\mappath{v_2}{p}}
\end{array}
\end{mathfig}

\caption{Path operations defined.}
\label{fig:paths}
\end{figure}


==> fig-prov-algebra.tex <==

\newcommand{\prov}[1]{\mathsf{P}\SB{#1}}
\newcommand{\preturn}[1]{\mathtt{return}~#1}
\newcommand{\pbind}{\mathrel{{>}\!\!{>}\!\!{=}}}
\newcommand{\provc}{\kwc^{P}}
\newcommand{\provf}[1]{\kwf^P(#1)}
\newcommand{\provpair}[2]{\mathtt{pair}^P(#1,#2)}
\newcommand{\provfst}[1]{\mathtt{fst}^P(#1)}
\newcommand{\provsnd}[1]{\mathtt{snd}^P(#1)}
\newcommand{\provinl}[1]{\mathtt{inl}^P(#1)}
\newcommand{\provinr}[1]{\mathtt{inr}^P(#1)}
\newcommand{\provcasel}[2]{\kwcase_{\mathtt{l}}^P(#1,#2)}
\newcommand{\provcaser}[2]{\kwcase_{\mathtt{r}}^P(#1,#2)}
\newcommand{\provroll}[1]{\kwroll^P(#1)}
\newcommand{\provunroll}[1]{\kwunroll^P(#1)}
\newcommand{\provfun}[2]{\kwfun^P(#1,#2)}
\newcommand{\provapp}[3]{\kwapp^P(#1,#2,#3)}
\newcommand{\plookup}[1]{\kw{lookup}^P~#1}
\newcommand{\pwith}{\mathrel{\kw{with}^P}}
\begin{figure}[p]
  \[\begin{array}{rcll}
\prov{e} &::& \prov{\Gamma} \to \prov{\tau}\\
   \prov{x} &=& \plookup{x}\\
   \prov{\exletin{x=e_1}{e_2}}\gamma &=& \prov{e_2} \pwith (x, \prov{e_1})\\
    \prov{\exc} &=& \preturn{c}\\
    \prov{\exf{e_1,\ldots,e_n}} &=&
    \prov{e_1} \pbind \lambda v_1.\\
&& \cdots\\
&& \prov{e_n} \pbind \lambda v_n.  \\
&&\preturn{\exf{v_1,\ldots,v_n}}\\
   \prov{\expair{e_1}{e_2}} &=&     \prov{e_1} \pbind \lambda v_1.\\
&& \prov{e_2} \pbind \lambda v_2.  \\
&&\preturn{(v_1,v_2)}\\
   \prov{\exfst{e}} &=& \prov{e} \pbind \lambda (v_1,v_2). \preturn{v_1}\\
    \prov{\exsnd{e}} &=& \prov{e} \pbind \lambda (v_1,v_2). \preturn{v_2}\\
    \prov{\exinl{e}} &=& \prov{e} \pbind \lambda v. \preturn{\exinl{v}}\\
    \prov{\exinr{e}} &=&  \prov{e} \pbind \lambda v. \preturn{\exinr{v}}\\
    \prov{\excasem{e}{m}} &=& \prov{e} \pbind
    \lambda v.\\
    && \kwcase~v~\kwof~\{
\\&&
\quad \kwinl(v_1).\preturn{\prov{e_1}[x_1\mapsto v_1]}
\\&& 
\quad \kwinr(v_2).\preturn{\prov{e_2}[x_2\mapsto  v_2]}
\\
&&\} \\
&&(\text{where } m = \match{x_1}{e_2}{x_2}{e_2})\\
   \prov{\exfunk{\kappa}}\gamma &=& \preturn{ \vclos{\kappa}{\gamma}}\\
    \prov{\exapp{e_1}{e_2}}\gamma &=& 
      \prov{e_1}\gamma \pbind \lambda \vclos{\fn{f}{x}{e}}{\gamma_0}.\\
     && \prov{e_2}\gamma \pbind \lambda v_2.\\
      &&\prov{e} \gamma_0[f \mapsto \vclos{\fn{f}{x}{e}}{\gamma_0}, x \mapsto v_2]\\
    \prov{\exroll{e}} &=& \prov{e} \pbind \lambda v. \preturn{\vroll{v}}\\
    \prov{\exunroll{e}} &=& \prov{e} \pbind  \lambda \vroll{v}.  \preturn{v}
 \end{array}\]
  \caption{Interpreting expressions in provenance monads}
  \label{fig:prov-alg}
\end{figure}


\begin{figure*}[p]
  \[\begin{array}{rcll}
    \prov{\tremp}\rho &=& \hole\\
    \prov{\trvar{x}}\rho &=& \rho(x)\\
   \prov{\trlet{T_1}{x}{T_2}}\rho &=& \prov{T_2}\rho[x:=\prov{T_1}\rho]\\
    \prov{\trc}\rho &=& \preturn{\provc}\\
    \prov{\trf{T_1,\ldots,T_n}}\rho &=&
    \prov{T_1}\rho \pbind \lambda p_1.\\
&& \cdots\\
&& \prov{T_n}\rho \pbind \lambda p_n.  \\
&&\preturn{\provf{p_1,\ldots,p_n}}\\
   \prov{\trpair{T_1}{T_2}}\rho &=&     \prov{T_1}\rho \pbind \lambda p_1.\\
&& \prov{T_2}\rho \pbind \lambda p_2.  \\
&&\preturn{\provpair{p_1}{p_2}}\\
   \prov{\trfst{T}}\rho &=& \prov{T}\rho \pbind \lambda p. \provfst{p}\\
    \prov{\trsnd{T}}\rho &=& \prov{T}\rho \pbind \lambda p. \provsnd{p}\\
    \prov{\trinl{T}}\rho &=& \prov{T}\rho \pbind \lambda p. \provinl{p}\\
    \prov{\trinr{T}}\rho &=&  \prov{T}\rho \pbind \lambda p. \provinr{p}\\
    \prov{\trcaseml{m}{T}{x_1}{T_1}}\rho &=& \prov{T}\rho \pbind \lambda \vinl{p}.\\
    && \provcasel{\prov{T}\rho}{\prov{T_1}\rho[x_1\mapsto p]}\\
   \prov{\trcasemr{m}{T}{x_2}{T_2}}\rho &=& \prov{T}\rho \pbind \lambda \vinr{p}.\\
    && \provcaser{\prov{T}\rho}{\prov{T_2}\rho[x_2\mapsto p]}\\
   \prov{\trfunk{\kappa}}\rho &=& \provfun{\kappa}{\rho}\\
    \prov{\trappk{\kappa}{T_1}{T_2}{f}{x}{T}}\rho &=& \provapp{\prov{T_1}{\rho}}{\prov{T_2}{\rho}}{\prov{T_3}\rho}\\
    \prov{\trroll{T}}\rho &=& \provroll{\prov{T}\rho}\\
    \prov{\trunroll{T}}\rho &=&  \provunroll{\prov{T}\rho}
 \end{array}\]
  \caption{Interpreting traces in provenance monads}
  \label{fig:prov-alg}
\end{figure*}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> fig-replay.tex <==
\begin{figure}[tb!]
\fbox{$\gamma,T \trrun v,T'$}
\vspace{-4mm}
\begin{smathpar}
\inferrule*
{
  \strut
}
{
  \gamma, \trvar{x} \trrun \gamma(x), \trvar{x}
}
\and
\inferrule*
{\strut}
{\gamma, \trc \trrun \exc, \trc}
\and
\inferrule*
{
  \strut
}
{
  \gamma,\trfunk{\kappa}
  \trrun 
  \vclos{\kappa}{\gamma}, \trfunk{\kappa}
}
\and
\inferrule*
{
  \gamma, \novec{T} \trrun \novec{v}, \novec{T'}
}
{
  \gamma, \trf{\novec{T}}
  \trrun 
  \hat{\oplus}(\novec{v}), \trf{\novec{T'}}
}
\and
\inferrule*
{
  \gamma,T_1 \trrun v_1,T_1'
\\
\gamma[x\mapsto v_1],T_2 \trrun v_2,T_2'
}
{
\gamma,\trlet{T_1}{x}{T_2} \trrun v_2,\trlet{T_1}{x}{T_2}
}
\and%
%
\inferrule*
{
 \gamma, T_1 \trrun v_{1}, T_1'
\\
 \gamma, T_2 \trrun v_{2}, T_2'
\\
}
{
  \gamma,  \trpair{T_1}{T_2}
  \trrun
  \vpair{v_{1}}{v_{2}}, \trpair{T_1'}{T_2'}
}
\and
%
\inferrule*
{
\gamma, T \trrun \vpair{v_{1}}{v_{2}}, T'
}
{
\gamma , \trfst{T} 
\trrun
v_{1} , \trfst{T'}
}
\and
%
\inferrule*
{
\gamma, T \trrun \vpair{v_{1}}{v_{2}}, T'
}
{
\gamma, \trsnd{T}
\trrun
v_2, \trsnd{T'}
}
%
\and
\inferrule*
{
  \gamma, T \trrun v, T'
}
{
\gamma, \trinl{T} \trrun \vinl{v}, \trinl{T'}
}
\and
\inferrule*
{
  \gamma, T \trrun v, T'
}
{
\gamma, \trinr{T} \trrun \vinr{v}, \trinr{T'}
}
\and
\inferrule*
{
\gamma, T \trrun \vinl{v}, T'
\\
\gamma[x_1 \mapsto v], T_1 \trrun v_1, T_1'
}
{
\gamma, \trcaseml{m}{T}{x_1}{T_1}
\trrun
v_1, \trcaseml{m}{T'}{x_1}{T_1'}
}
\and 
\inferrule*
{
\gamma, T \trrun \vinr{v}, T'
\\
\gamma[x_2 \mapsto v], T_2 \trrun v_2, T_2'
}
{
\gamma, \trcasemr{m}{T}{x_2}{T_2}
\trrun
v_2, \trcasemr{m}{T'}{x_2}{T_2'}
}
\and
\inferrule*
{
\gamma,T_1 \trrun \vclos{\kappa}{\gamma'},T_1'
\\
\gamma,T_2 \trrun v_2,T_2'
\\
\gamma'[f\mapsto\vclos{\kappa}{\gamma'}, x\mapsto v_2],T \trrun v,T'
}
{
\gamma,\trappk{\kappa}{T_1}{T_2}{f}{x}{T} \trrun v,\trappk{\kappa}{T_1'}{T_2'}{f}{x}{T'}
}
\and
\inferrule*
{
  \gamma, T \trrun v, T'
}
{
\gamma, \trroll{T} \trrun \vroll{v}, \trroll{T'}
}
\and
\inferrule*
{
  \gamma, T \trrun \vroll{v}, T'
}
{
\gamma, \trunroll{T} \trrun {v}, \trunroll{T'}
}
\and
\inferrule*[Right=($\dagger$1)]
{
\kwinl(x_2).e_2 \in m
\\
\gamma, T \trrun \vinr{v}, T'
\\
\gamma[x_2 \mapsto v], e_2 \red v_2, T_2'
}
{
\gamma, \trcaseml{m}{T}{x_1}{T_1}
\trrun
v_2, \trcasemr{m}{T'}{x_2}{T_2'}
}
\and
%
\inferrule*[Right=($\dagger$2)]
{
\kwinr(x_1).e_1 \in m
\\
\gamma, T \trrun \vinl{v}, T'
\\
\gamma[x_1 \mapsto v], e_1 \red v_1, T_1'
}
{
\gamma, \trcasemr{m}{T}{x_2}{T_2}
\trrun
v_1, \trcaseml{m}{T'}{x_1}{T_1'}
}
\and
\inferrule*[Right=($\dagger$3)]
{
T_1 \trrun \vclos{\kappa'}{\gamma'},T_1'
\\
(\kappa' = \exfun{f}{x}{e'} \neq \kappa)
\\
T_2 \trrun v_2,T_2'
\\
\gamma'[f\mapsto \vclos{\kappa'}{\gamma'}, x\mapsto v_2] , e' \red v', T_3'
}
{
\gamma, \trappk{\kappa}{T_1}{T_2}{f}{x}{T_3} \trrun v', \trappk{\kappa'}{T_1'}{T_2'}{f}{x}{T_3'}
}
% \and
% \inferrule*
% {\strut}
% {\gamma, \tremp \trrun \vhole, \tremp}
\end{smathpar}
\caption{Dynamic semantics of $\plz$: trace replay.}
\label{fig:replay}
\end{figure}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> fig-slice-better.tex <==
\begin{figure}[tb!]
\begin{smathpar}
  \inferrule*
  {
    p, T \bwdslice S, \rho[f \mapsto \vclos{\fn{f}{x}{e_0}}{\rho_0}, x \mapsto p_2]
    \\
    p, T \bwdpslice e, \_
    \\
    \vclos{\fn{f}{x}{(e \sqcup e_0)}}{\rho \sqcup \rho_0}, T_1 \bwdslice S_1,\rho_1
    \\
    p_2,T_2 \bwdslice S_2,\rho_2     }
  {
    p, \trappk{\kappa}{T_1}{T_2}{f}{x}{T} 
    \bwdslice 
    \trappk{\kappa}{S_1}{S_2}{f}{x}{S} ,\rho_1 \sqcup \rho_2
  }
\end{smathpar}
%\hrule
\caption{Alternative trace slicing rule for function bodies, making use of unevaluation.}
\label{fig:traceslice-better}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-slices-defined.tex <==

\begin{figure}[tb]
\fbox{$T\sqleq T'$}
\vspace{-4mm}
\begin{smathpar}
     \inferrule
      {\strut}
      {\tremp \sqleq T}
\and
%
   \inferrule {\strut} {\trc \sqleq \trc} 
    % 
    \and
    %
    \inferrule {\novec{T} \sqleq \novec{T}'} {\trf{\novec{T}} \sqleq
      \trf{\novec{T}'}}
    % 
    \and 
    % 
    \inferrule { \strut } { \trvar{x} \sqleq \trvar{x} } 
    % 
    \and
%
    \inferrule {
      T_1 \sqleq  T_1'\\
      T_2 \sqleq T_2' } { \trlet{T_1}{x}{T_2} \sqleq
      \trlet{T_1'}{x}{T_2'} } 
%
\and 
%
\inferrule {
      T_1 \sqleq T_1' \\
      T_1 \sqleq T_2' } { \trpair{T_1}{T_2} \sqleq \trpair{T_1'}{T_2'}
    } 
%
\and 
%
\inferrule { T \sqleq T' } { \trfst{T} \sqleq \trfst{T'} }
%
    \and 
%
\inferrule { T \sqleq T' } { \trsnd{T} \sqleq \trsnd{T'} }
%
    \and 
%
\inferrule{T \sqleq T' }{\trinl{T} \sqleq \trinl{T'}}
%
 \and
%
    \inferrule{T \sqleq T' }{\trinr{T} \sqleq \trinr{T'}}
%
\and
   \inferrule
      {
        T \sqleq T'
        \\
        T_1 \sqleq T_1'
      }
      {
        \trcaseml{m}{T}{x}{T_1} \sqleq \trcaseml{m}{T'}{x}{T_1'}
      }
      \and
   \inferrule
      {
        T \sqleq T'
        \\
        T_2 \sqleq T_2'
      }
      {
        \trcasemr{m}{T}{x}{T_2} \sqleq \trcasemr{m}{T'}{x}{T_2'}
      }
      \and    
     \inferrule
      {
        \kappa \sqleq \kappa'
      }
      {
        \trfunk{\kappa} \sqleq \trfunk{\kappa'}
      }     
       \and
      \inferrule
      {
        \kappa \sqleq \kappa'\\
        T_1 \sqleq T_1'\\
        T_2 \sqleq T_2'\\
        T \sqleq T'
      }
      {
        \trappk{\kappa}{T_1}{T_2}{f}{x}{T} \sqleq \trappk{\kappa'}{T_1'}{T_2'}{f}{x}{T'} 
      }
%
       \and 
%
        \inferrule{T \sqleq T' }{\trroll{T} \sqleq \trroll{T'}}
%
        \and
%
        \inferrule{T \sqleq T' }{\trunroll{T} \sqleq \trunroll{T'}}
\end{smathpar}
%\hrule
\caption{Judgments for partial traces.}
\label{fig:slices-defined}
\end{figure}
\begin{figure}[tb]
\fbox{$v \eqat{p} v$}
\vspace{-3mm}
\begin{smathpar}
\inferrule*{
\strut
}
{v \eqat{\vhole} v'}
\and
\inferrule*
{
\strut
}
{
v \eqat{\vany} v
}
\and
\inferrule*
{
\strut
}
{
\vc \eqat{\vc} \vc
}
\and
\inferrule*
{
  v_1 \eqat{p_1} v_1'
  \\
  v_2 \eqat{p_2} v_2'
}
{
  \vpair{v_1}{v_2} \eqat{(p_1,p_2)} \vpair{v_1'}{v_2'}
}
\and
\inferrule*{v \eqat{p} v'}
{\vinl{v} \eqat{\vinl{p}} \vinl{v'}}
\and
\inferrule*{v \eqat{p} v'}
{\vinr{v} \eqat{\vinr{p}} \vinr{v'}}
\and
\inferrule*{v \eqat{p} v'}
{\vroll{v} \eqat{\vroll{p}} \vroll{v'}}
\and
\inferrule*{
\kappa \eqat{\kappa_0} \kappa'\\
\gamma \eqat{\rho}\gamma'
}
{
\vclos{\kappa}{\gamma} \eqat{\vclos{\kappa_0}{\rho}} \vclos{\kappa'}{\gamma'}
}
\end{smathpar}
\begin{eqnarray*}
  \gamma \eqat{\rho} \gamma' &\iff &\forall x \in
  \dom(\rho). ~\gamma(x) \eqat{\rho(x)} \gamma'(x)
%\\
 % \gamma \eqat{\vany} \gamma' &\iff & \gamma = \gamma'\\
 % \gamma \eqat{\vhole} \gamma'& \iff &\top
\end{eqnarray*}
\fbox{$p \sqleq p'$}
\vspace{-3mm}
\begin{smathpar}
\inferrule*{\strut}{\vhole\sqleq p}
\and
\inferrule*{\text{no $\vhole$s in $p$}}{\vany\sqleq p}
\and
\inferrule*{
  p_1 \sqleq p_1' \\ 
  p_2 \sqleq p_2'
}{
  \vpair{p_1}{p_2} \sqleq \vpair{p_1'}{p_2'}
}
\and
\inferrule*{
  p \sqleq p' 
}{
  \vinl{p} \sqleq \vinl{p'}
}
\and
\inferrule*{
  p \sqleq p '
}{
  \vinr{p} \sqleq \vinr{p'}
}
\and
\inferrule*{
  p \sqleq p'
}{
  \vroll{p} \sqleq \vroll{p'}
}
\and
\inferrule*
{
\kappa \sqleq \kappa' \\
  \rho \sqleq \rho'
}
{
  \vclos{\exfunk{\kappa}}{\rho} \sqleq \vclos{\exfunk{\kappa'}}{\rho'}
}
\and
\rho \sqleq \rho' \iff 
  \forall x \in \dom(\rho). ~\rho(x) \sqleq \rho'(x)
\end{smathpar}
%\hrule
\caption{Equality modulo patterns; pattern containment.}
\label{fig:patterns}
\[\small \begin{array}{rcl}
    \vhole \sqcup p = p \sqcup \vhole &=& p \qquad 
    \vany \sqcup p = p \sqcup \vany = p[\vany/\vhole]\\[1mm]
   \vpair{p_1}{p_2} \sqcup \vpair{p_1'}{p_2'} &=& \vpair{p_1\sqcup
      p_1'}{p_2\sqcup p_2'} \qquad 
 c \sqcup c = c \\[1mm]
    C(p) \sqcup C(p') &=& C(p\sqcup p') \qquad C \in \{\kwinl,\kwinr,\kwroll\}\\[1mm]
\vclos{\kappa}{\rho} \sqcup \vclos{\kappa'}{\rho'} &=& \vclos{\kappa
  \sqcup \kappa'}{\rho \sqcup \rho'}\\[1mm]
    (\rho \sqcup \rho')(x) &=& \left\{
      \begin{array}{ll}
        \rho(x) \sqcup \rho'(x) & x \in \dom(\rho) \cup \dom(\rho')\\
        \rho(x) & x \in \dom(\rho) \backslash \dom(\rho')\\
        \rho'(x) & x \in \dom(\rho') \backslash \dom(\rho)
     \end{array}\right.
 \end{array}\]
\caption{Least upper bounds of patterns and environments.}
\label{fig:pattern-lub}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-syn-trace.tex <==
\begin{figure}[t]
\begin{syntaxfig}
\mbox{Traces}
& 
T
& 
::=
& 
\trvar{x}
\mid 
\trlet{T_1}{x}{T_2}
\mid
\trc 
\mid 
\trf{\novec{T}}
\\[1mm]
&
& 
\mid
& 
\trpair{T_1}{T_2}
\mid
\trfst{T}
\mid
\trsnd{T}
\\[1mm]
&&\mid& 
\trinl{T}
\mid 
\trinr{T}
\\[1mm]
&
& 
\mid
& 
\trcaseml{m}{T}{x}{T_1}
\mid
\trcasemr{m}{T}{x}{T_2}
\\[1mm]
&&
\mid 
&
\trfunk{\kappa}
\mid
\trappk{\kappa}{T_1}{T_2}{f}{x}{T}
\\[1mm]
&& 
\mid &
\trroll{T} \mid \trunroll{T}
\end{syntaxfig}
\caption{Abstract syntax for traces.}
\label{fig:syn}
\end{figure}


==> fig-syn.tex <==
\begin{figure}[t]
\begin{syntaxfig}
\mbox{Types}
&
\tau
& 
::=
& 
b
\mid
% \kwbool
% \mid
\tau_1 \times\tau_2
\mid
\tau_1 + \tau_2
\mid
\tau_1 \ra \tau_2
\mid 
\tyrec{\alpha}{\tau}
\mid 
\alpha
\\[1mm]
\mbox{Type contexts}
&
\Gamma 
&
::= &
[x_1:\tau_1 , \ldots , x_n:\tau_n]
\\[1mm]

\mbox{Code pointers}
  &
  \kappa
  & 
  ::= 
  &
  \vclos{\fn{f}{x}{e}}{\Gamma}
  \\[1mm]

\mbox{Matches}
  &
  m
  & 
  ::= 
  &
  \match{x_1}{e_1}{x_2}{e_2}
  \\[1mm]
 % 



 \mbox{Values}
  &
  v
  & 
  ::=
  & 
  \vc
  \mid
  \vpair{v_1}{v_2}
  \mid 
  \vinl{v}
  \mid 
  \vinr{v}
  \mid
  \vclos{\kappa}{\gamma}
  \mid 
  \vroll{v}
 \\[1mm]
%
  \mbox{Expressions}
  & 
  e,T
  & 
  ::=
  & 
   \exc 
  \mid
  x
  \mid  
\exf{\novec{e}}
 \mid
  \exletin{x=e_1}{e_2} 
\\[1mm]
&&\mid
&  \expair{e_1}{e_2}
  \mid
  \exfst{e}
  \mid
  \exsnd{e}
  \\[1mm]
&&\mid
&
  \exroll{e}
  \mid
  \exunroll{e}
  \\[1mm]
  &
  & 
  \mid
  & 
  \exinl{e}
  \mid
  \exinr{e}
  \mid
 \exfunk{\kappa} 
\mid
  \excasem{e}{m}
  \mid
  \exapp{e}{e'}
  \\[2mm]
&&\mid& 
\trcaseml{m}{T}{x}{T_1}
\\[1mm]
&&\mid& 
\trcasemr{m}{T}{x}{T_2}
\\[1mm]
&&\mid& 
\trappk{\kappa,\Gamma}{T_1}{T_2}{f}{x}{T} 
% 
\\[1mm]
 % 
\mbox{Environments}
&
\gamma 
& 
::= 
& 
[x_1 \mapsto v_1,\ldots,x_n \mapsto v_n]
\begin{tronly}
  \\[1mm]
  \mbox{Traces} & T & ::= & \trvar{x} \mid \trlet{T_1}{x}{T_2} \mid
  \trc \mid \trf{\novec{T}}
  \\[1mm]
  &&\mid& \trpair{T_1}{T_2} \mid \trfst{T} \mid \trsnd{T}
  \\[1mm]
  &&\mid& \trinl{T} \mid \trinr{T}
  \\[1mm]
  &&\mid& \trcaseml{m}{T}{x}{T_1} \mid \trcasemr{m}{T}{x}{T_2}
  \\[1mm]
  && \mid & \trfunk{\kappa} \mid \trappk{\kappa,\Gamma}{T_1}{T_2}{f}{x}{T}
  \\[1mm]
  &&\mid& \trroll{T} \mid \trunroll{T}
\end{tronly}
\end{syntaxfig}
\caption{Abstract syntax of $\plz$.}
\label{fig:syn}
\end{figure}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 
 


==> fig-unevaluation.tex <==
\begin{figure}[tb!]
\fbox{$T \uneval e$}
\begin{smathpar}
\inferrule*
{
}
{
  \tremp \uneval \hole
}
\and
\inferrule*
{
}
{
  \trcon{c} \uneval \kwc
}
\and
\inferrule*
{
}
{
  \trvar{x} \uneval x
}
\and
\inferrule*
{
}
{
\trfunk{\kappa} \uneval \exfunk{\kappa}
}
\and
\inferrule*
{
T_1 \uneval e_1 \\
T_2 \uneval e_2
}
{
\trlet{T_1}{x}{T_2} \uneval \exlet{x}{e_1}{e_2}
}
\and
\inferrule*
{
T_1 \uneval e_1 \\
\cdots \\
T_n \uneval e_n
}
{
\trf{T_1,\ldots,T_n} \uneval \exf{e_1,\ldots,e_n}
}
\and
\inferrule*
{
  T_1 \uneval e_1 \\
  T_2 \uneval e_2
}
{
\trpair{T_1}{T_2} \uneval \expair{e_1}{e_2}
}
\and
\inferrule*
{
T \uneval e
}
{
\trfst{T} \uneval \exfst{e}
}
\and
\inferrule*
{
T \uneval e
}
{
\trsnd{T} \uneval \exsnd{e}
}
\and
\inferrule*
{
T \uneval e
}
{
\trinl{T} \uneval \exinl{e}
}
\and
\inferrule*
{
T \uneval e
}
{
\trinr{T} \uneval \exinr{e}
}
\and
\inferrule*
{
T \uneval e \\
T_1 \uneval e_1
}
{
\trcaseml{m}{T}{x}{T_1} \uneval \excase{e}{x_1}{e_1}{x_2}{\hole}
}
\and
\inferrule*
{
T \uneval e\\
T_2 \uneval e_2
}
{
\trcasemr{m}{T}{x}{T_2} \uneval \excase{e}{x_1}{\hole}{x_2}{e_2}
}
\and
\inferrule*
{
T_1 \uneval e_1\\
T_2 \uneval e_2
}
{
\trappk{\kappa}{T_1}{T_2}{f}{x}{T} \uneval \exapp{e_1}{e_2}
}
\and
\inferrule*
{
T \uneval e
}
{
\trroll{T} \uneval \exroll{e}
}
\and
\inferrule*
{
T \uneval e
}
{
\trunroll{T} \uneval \exunroll{e}
}
\end{smathpar}
\caption{The unevaluation algorithm.}
\label{fig:unevaluation}

\begin{smathpar}
  \inferrule*
  {
  }
  {
    \vclos{\kappa}{\rho}, \trfunk{\kappa_0} \bwdslice \trfunk{\kappa},\rho
  }
  \and
  \inferrule*
  {
    p, T \bwdslice S, \rho[f \mapsto \vclos{\fn{f}{x}{e_0}}{\rho_0}, x \mapsto p_2]
    \\
    S \uneval e
    \\
    \vclos{\fn{f}{x}{(e \sqcup e_0)}}{\rho \sqcup \rho_0}, T_1 \bwdslice S_1,\rho_1
    \\
    p_2,T_2 \bwdslice S_2,\rho_2     }
  {
    p, \trappk{\kappa}{T_1}{T_2}{f}{x}{T} 
    \bwdslice 
    \trappk{\kappa}{S_1}{S_2}{f}{x}{S} ,\rho_1 \sqcup \rho_2
  }
\end{smathpar}
\caption{Rules for unevaluation during slicing}
\label{fig:unevaluation-slicing}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> fig-where.tex <==
\begin{figure}[tb]
  \[\small\begin{array}{rcll}
   \where(\exvar{x},\agamma) &=& \agamma(x)\\[1pt]
    \where (\exlet{e_1}{x}{e_2},\agamma) &=& \where(e_2,\agamma[x\bindsto \where(e_1,\agamma)])\\[1pt]
    \where (\exc,\agamma) &=&\exc^\bot\\[1pt]
    \where (\exf{e_1,\ldots,e_n},\agamma) &=&
    (\hat{f}(v_1,\ldots,v_n))^\bot
    \\&\text{where}&v_i^{a_i} = \where(e_i,\agamma)\\[1pt]
    \where (\expair{e_1}{e_2},\agamma) &=& (\where(e_1,\agamma),\where(e_2,\agamma))^\bot\\[1pt]
    \where (\exfst{e},\agamma) &=& v_1
    \\&\text{where}& (v_1,v_2)^a = \where(e,\agamma)\\[1pt]
    \where (\exsnd{e},\agamma) &=&  v_2 
    \\&\text{where}& (v_1,v_2)^a = \where(e,\agamma)\\[1pt]
    \where (\exinl{e},\agamma) &=& \vinl{\where(e,\agamma)}^\bot\\[1pt]
    \where (\exinr{e},\agamma) &=&  \vinr{\where(e,\agamma)}^\bot\\ [1pt]
    \where (\excasem{e}{m},\agamma) &=& \where
   (e_1,\agamma[x\bindsto v])
  \quad\text{where}\vinl{v}^a = \where(e,\agamma),\\
&&  \kwinl(x_1).e_1 \in m\\[1pt]
 \where (\excasem{e}{m},\agamma) &=& \where
    (e_2,\agamma[y\bindsto v])
    \\&\text{where}& \vinr{v}^a = \where(e,\agamma),\\
&&  \kwinr(x_2).e_2 \in m\\[1pt]
    \where (\exfunk{\kappa},\agamma) &=& (\Lambda
    \av.~ \where\SB{e}\agamma[x\bindsto \av])^\bot\\[1pt]
%     \where (\exappk{e_1}{e_2},\agamma) &=&  \where(e_3,\agamma'[f\bindsto
%     \vclos{\kappa}{\agamma'}^a, x \bindsto v_2]) 
%     \\&\text{where}&\vclos{\kappa}{\agamma'}^a =
%     \where(e_1,\agamma),
%     \\&& v_2 =\where(e_2,\agamma) \\[1pt]
    \where (\exroll{e},\agamma) &=& \vroll{\where(e,\agamma)}^\bot\\[1pt]
    \where (\exunroll{e},\agamma) &=&  v 
    \\&\text{where}& \vroll{v}^a = \where(e,\agamma)
 \end{array}\]
  \caption{Where-provenance extraction.}
  \label{fig:where-from-trace}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> further-examples.tex <==
\section{Concrete syntax for traces and trace slices}
\label{app:further-examples}

\input{fig-example-merge-1}
\input{fig-example-merge-2}

\figref{example-merge-1} shows a program which merges two sorted lists of integers. In \figref{example-merge-2}, we show the trace of the program after it has been sliced with a pattern which picks out the last element of the output list.

The trace syntax employed here makes use of a number of typographical conventions, not all of which are relevant to expressions. Binding occurences of variables are underlined, to distinguish them from uses. Constructor names that occur in the constructor patterns of taken branches are highlighted in magenta; the not-taken branches are simply omitted. (Booleans are primitive here, rather than a datatype, which is why \Verb|if| expressions are not presented similarly.) Finally, the function expression in an application trace, which is often simply an identifier, is highlighted in blue. These conventions are not essential, but improve readability.

Aside from the omitted case-branches, the main structural difference between a trace and a program is that applications are expanded inline, showing the new binding occurrences of the function parameters, the token ``\Verb|=>|'' to echo the expression syntax for functions, and then the trace of the function body. In an editor this inline expansion could be driven interactively by the user.

The example also illustrates how higher-order values are sliced in the presence of recursion. At the top of the trace in \figref{example-merge-2}, we see the let-variable \Verb|merge| being bound to the definition of a recursive function of the same name. After slicing, this functional value has been sliced in a way that reflects its usage in the computation. Both \Verb|Nil| branches have been replaced with a hole, indicating that the end of neither input list was reached. The hole in the head position of the first \Verb|Cons| operation reflects the fact that \Verb|13| was picked from the second list, not the first.

==> ldefs.tex <==
%% Language
\newcommand{\lang}{\mbbl\xspace}
\newcommand{\lvars}{\mcx\xspace}
\newcommand{\lexps}{\mce\xspace}
\newcommand{\lvals}{\mcv\xspace}
\newcommand{\ltrs}{\mct\xspace}
\newcommand{\lbls}{\mcl\xspace}

% 
\newcommand{\nrc}{\mbox{\textsf{NRC}}}

% Types
\newcommand{\tyint}{\im{\kw{int}}}
\newcommand{\tybool}{\im{\kw{bool}}}

% semantic operators
\newcommand{\semplus}{\im{\,\hat{+}\,}}
\newcommand{\semeq}{\im{\,\hat{=}\,}}
\newcommand{\semu}{\im{\,\hat{\cup}\,}}

% substitution
\newcommand{\subst}[3]{{#3}[{#1}/{#2}]} 
\newcommand{\sub}[3]{{#3}[{#1}/{\{#2\}}]}

% eval
\newcommand{\leval}{\im{\Downarrow}\xspace}

% contexts
\newcommand{\ctxe}{\im{\bullet}}

\newcommand{\dctx}{\im{\bigtriangledown}}

% labels
\newcommand{\bindl}[2]{\im{{#1}.{#2}}}
\newcommand{\lbl}{\im{\ell}\xspace}
\newcommand{\lbla}{\im{{\ell_1}}\xspace}
\newcommand{\lblaa}{\im{{\ell_{11}}}\xspace}
\newcommand{\lblb}{\im{{\ell_{2}}}\xspace}
\newcommand{\lblbb}{\im{{\ell_{22}}}\xspace}
\newcommand{\lblc}{\im{{\ell_3}}\xspace}
\newcommand{\lblcc}{\im{{\ell_{33}}}\xspace}
\newcommand{\lblsOf}[1]{\im{\kw{labelsOf}({#1})}}
\newcommand{\expAt}[2]{\im{{#1}[{#2}]}}
\newcommand{\toplbls}[1]{\im{\kw{toplabels}({#1})}}

%$ Provenance System
\newcommand{\pfun}{\im{\phi}\xspace}

\newcommand{\pfunb}{\im{\phi_b}\xspace}
\newcommand{\pfunf}{\im{\phi_f}\xspace}
\newcommand{\treval}{\im{\ca}}
\newcommand{\coneval}{\im{\ca}}
%\newcommand{\ps}[3]{\im{({#1},{#2},{#3})}}
\newcommand{\ps}[4]{\im{({#1},({#2},{#3}),{#4})}}
\newcommand{\pins}{\mbbp\xspace}

%% Types
\newcommand{\kwbool}{\im{\kw{bool}}}
\newcommand{\kwb}{\im{\kw{b}}}
%% Terms

\newcommand{\kwnone}{\im{\kw{NONE}}}
\newcommand{\kwsome}[1]{\im{\kw{SOME}~{#1}}}
\newcommand{\kwtrue}{\im{\kw{true}}}
\newcommand{\kwfalse}{\im{\kw{false}}}
\newcommand{\kwc}{\im{\kw{c}}}
\newcommand{\kwf}{\im{\kw{f}}}
\newcommand{\kwn}{\im{\kw{n}}}
\newcommand{\kwpair}[2]{\im{({#1},{#2})}}
\newcommand{\kwfst}[1]{\im{\kw{fst}~{#1}}}
\newcommand{\kwsnd}[1]{\im{\kw{snd}~{#1}}}
\newcommand{\kwlam}[3][]{\im{\lambda ^{#1}{#2}.{#3}}}
\newcommand{\kwif}[3]{\im{\kw{if}~{#1}~\kw{then}~{#2}~\kw{else}~{#3}}}
\newcommand{\kwsete}{\im{\emptyset}}
\newcommand{\kwset}[1]{\im{\set{#1}}}
\newcommand{\kwsets}[1]{\im{\set{#1}}}
\newcommand{\kwsetu}[2]{\im{{#1} \cup {#2}}}
\newcommand{\kwsetise}[1]{\im{\kw{empty}~{#1}}}
\newcommand{\kwsetcomp}[3]{\im{\set{{#1\!}\mid{#2 \in #3}}}}
\newcommand{\kwlet}[3]{\im{\kw{let}~{#1}\:=\:{#2}~\kw{in}~{#3}}}
\newcommand{\kwapp}[2]{\im{{#1}~{#2}}}
\newcommand{\kwsum}[1]{\im{\kw{sum}~{#1}}}
%\newcommand{\kwsum}[1]{\im{\sum {#1}}}
\newcommand{\kwflatten}[1]{\im{\bigcup {#1}}}

% no longer used(?)
\newcommand{\kwsetsel}[1]{\im{\kw{select}~{#1}}}
\newcommand{\kwsetm}[2]{\im{\set{{#1}~\mid~{#2}}}}
\newcommand{\kwfun}[3]{\im{\kw{fun}~{#1}.{#2}.{#3}}}
\newcommand{\kwsetr}[2]{\im{\kw{reduce}~{#1}~{#2}}}


%% Traces
\newcommand{\sli}{\sqsubseteq}
\newcommand{\trsub}{\sqsubseteq}
\newcommand{\trlub}{\sqcup}
\newcommand{\trred}{\downarrow}
\newcommand{\trslice}[1][]{\stackrel{#1}{\leadsto}}
\newcommand{\trbslice}{\searrow}
\newcommand{\trfslice}{\nearrow}
\newcommand{\sliceof}{\hole}
\newcommand{\trhole}{\hole}

\newcommand{\tremp}{\im{\hole}}
%\newcommand{\mktrace}[1]{\im{\langle {#1} \rangle}}
\newcommand{\mktrace}[1]{\im{{#1}}}
\newcommand{\trv}[1]{\mktrace{#1}}
\newcommand{\trlbl}[2]{\mktrace{\bindl{#1}{#2}}}
\newcommand{\trpair}[2]{\mktrace{\kwpair{#1}{#2}}}
\newcommand{\trsetise}[1]{\kw{empty}~{#1}}
\newcommand{\trsets}[2]{\{\trlbl{#1}{#2}\}}
\newcommand{\trsetu}[2]{\mktrace{{#1}~\cup~{#2}}}
\newcommand{\trbindl}[3]{\mktrace{{#1}\:\kw{in}\:{#2} . {#3}}}
\newcommand{\trbindlt}[2]{\mktrace{{#1}\:\kw{in}\:{#2}}}
\newcommand{\trsetcomp}[4]{\mktrace{\set{{#1}~\kw{with}~{#3}.{#4}~\mid~{#2}}}}
\newcommand{\trplus}[2]{\mktrace{{#1} + {#2}}}
\newcommand{\trsum}[2]{\mktrace{{#1} + {#2}}}
\newcommand{\treq}[2]{\mktrace{{#1} = {#2}}}
\newcommand{\trfst}[1]{\mktrace{{\kw{fst}}~#1}}
\newcommand{\trsnd}[1]{\mktrace{{\kw{snd}}~#1}}
\newcommand{\trif}[3]{\mktrace{{\kw{if}}~{#1}~{\kw{then}}~{#2}~{\kw{else}}~{#3}}}
\newcommand{\trifthen}[2]{\mktrace{{\kw{if}}~{#1}~{\kw{then}}~{#2}}}
\newcommand{\trifelse}[2]{\mktrace{{\kw{if}}~{#1}~{\kw{else}}~{#2}}}
\newcommand{\trlet}[3]{\mktrace{{\kw{let}}~{#1} = {#2}~\kw{in}~{#3}}}
\newcommand{\trsetsum}[1]{\mktrace{\kwsum{#1}}}
\newcommand{\trflatten}[1]{\mktrace{\kwflatten{#1}}}
\newcommand{\trlet}[2]{\mktrace{{\kw{let}}({#1},{#2})}}
\newcommand{\trapp}[5]{\mktrace{{\kw{app}}^{#1}({#2},{#4},{#5})}}
\newcommand{\trcache}[2]{\langle #1 \rangle_{#2}}
\newcommand{\trrun}{\im{\curvearrowright}}

% running comprehension traces: 
\newcommand{\trruncomp}[5]{{#1},\,{#2},\,{#3} . {#4} \trrun^\star {#5}}
\newcommand{\trbindlmap}[3]{\mktrace{{#1}\mapsto{#2} . {#3}}}

% following should be removed
\newcommand{\trsetm}[3]{\mktrace{\set{{#1} = {#2}~|~ {#3}}}}
\newcommand{\trsetsel}[2]{\kw{select}~{#1}~{#2}}



%% Paths
\newcommand{\pe}{\im{\varepsilon}}
\newcommand{\pcons}[2]{\im{{#1} \cdot {#2}}}

\newcommand{\atpath}[2]{\im{{#1} \,@\, {#2}}}
\newcommand{\mappath}[2]{\im{{#1} \curlyvee {#2}}}

% Similarity
\newcommand{\simx}[1]{\im{\stackrel{#1}{\sim}}}
\newcommand{\expsim}[3]{\im{{#1}~\sim~{#2}}}
% similar at p:
\newcommand{\simat}[1]{\eqat{#1}}
%equal at p
\newcommand{\eqat}[1]{\im{\approx_{#1}}}


\newcommand{\dom}{\mathrm{dom}}

\newcommand{\SB}[1]{\llbracket #1 \rrbracket}

\newcommand{\paths}[1]{\im{\mathit{paths}({#1})}}
\newcommand{\Deriv}{\mathit{Deriv}}
\newcommand{\ext}[1]{\stackrel{#1}{\to}}
\newcommand{\wext}{\stackrel{W}{\to}}
\newcommand{\qext}{\stackrel{Q}{\to}}
\newcommand{\sqleq}{\sqsubseteq}

\newenvironment{mathfig}{\begin{sdisplaymath}}{\end{sdisplaymath}}
\newenvironment{syntaxfig}{\begin{mathfig}\begin{array}{@{}l@{\quad}r@{~~}c@{\quad}l}}{\end{array}\end{mathfig}}

\newcommand{\Pow}[1]{\mathcal{P}({#1})}
\newcommand{\where}{\mathsf{W}}
\newcommand{\dep}{\mathsf{D}}
\newcommand{\expr}{\mathsf{E}}
\newcommand{\extract}{\mathsf{F}}
\newcommand{\trace}{\mathsf{T}}

\newcommand{\Slice}{\mathsf{Slice}}
\newcommand{\RSlice}{\mathsf{RSlice}}
\newcommand{\MinRSlice}{\mathsf{MinRSlice}}
\newcommand{\CSlice}{\mathsf{CSlice}}
\newcommand{\MinCSlice}{\mathsf{MinCSlice}}
\newcommand{\fslice}{\mathsf{F_{min}}}
\newcommand{\bslice}{\mathsf{B_{min}}}
\newcommand{\BSlice}{\mathsf{BSlice}}
\newcommand{\FSlice}{\mathsf{FSlice}}
\newcommand{\Trace}{\mathsf{Trace}}
\newcommand{\Path}{\mathsf{Path}}
\newcommand{\Lab}{\mathsf{Lab}}

\newcommand{\abstr}[2]{{#1}\backslash{#2}}


\renewcommand{\vec}[1]{\overline{#1}}
\newcommand{\novec}[1]{#1}


==> patterns.tex <==
\section{Patterns, partial traces, and trace queries}


\highlight{In Section~\ref{sec:extraction}, we introduced several
  formalisms for provenance as instances of a generic framework.
  Earlier inthe paper, in section ~\ref{sec:background}, we reviewed
  and refined a general provenance framework with definitions of
  disclosure and obfuscation.  In this section, we introduce
  additional comcepts needed to formulate the \pl model of provenance
  as an instance of the abstract provenance framework, so that we can
  analyze the security propertis of \pl traces.  Specifically, we will
  consider a consistent triple $(gamma,T,v)$ as an abstract trace, we will define some provenance queries over such traces, and we will consider some approaches to defining provenance views of the traces.  The queries and views rely on notions of patterns and partial traces; specifically, we will consider queries based on testing whether a partial value is present in the input or output,and we will consider views based on deleting information from the trace, input or output.  }

We introduce patterns for values, environments and traces.  The syntax
of patterns (pattern environments) is similar to that of values
(respectively environments), extended with special \emph{holes}:
\begin{eqnarray*}
  p &::=& \vc \mid \vpair{p_1}{p_2} \mid \vinl{p} \mid \vinr{p} \mid
  \vroll{p} \mid \vclos{\kappa}{\rho} \mid \vany \mid \vhole
\\
\rho &::=& [x_1 \mapsto p_1,\ldots,x_n \mapsto p_n]
\end{eqnarray*}
Patterns actually denote binary relatidons on values.  The hole symbol
$\vhole$ denotes the total relation, while the exact-match symbol
$\vany$ denotes the identity relation.  The $\vany$ pattern is a
technical device used later in backward disclosure slicing (see
Section \ref{sec:analysis}; we
sometimes refer to \emph{$\vany$-free patterns} that do not contain
$\vany$.

We say that $v$ matches $v'$ modulo $p$ (written $v \eqat{p} v'$) if
$v$ and $v'$ match the structure of $p$, and are equal at
corresponding positions denoted by $\vany$.  Moreover, we write $p
\sqcup p'$ for the least upper bound (join) of two patterns and define
$p \sqleq p'$ to hold if $p' = p \sqcup p'$.  Rules defining
$\eqat{p}$ and $\sqcup$ are given in Figures~\ref{fig:eqat}
and~\ref{fig:lub}.  In the equations defining $p \sqcup
\vany$, we use notation $p[\vany/\vhole]$ to denote the result of
replacing all occurrences of $\vhole$ in $p$ with $\vany$.

When $p \sqsubseteq v$, we write $v|_p$ for the pattern obtained by
replacing all of the $\vany$-holes in $p$ with the corresponding
values in $v$, defined as follows:
\begin{eqnarray*}
  v|_\vhole &=& \vhole\\
v|_\vany &=& v\\
\vc|_\vc &=& \vc\\
(v_1,v_2)|_{(p_1,p_2)} &=& (v_1|_{p_1},v_2|_{p_2})\\
\vinl{v}|_{\vinl{p}} &=& \vinl{v|_p}\\
\vinr{v}|_{\vinr{p}} &=& \vinr{v|_p}\\
\vroll{v}|_{\vroll{p}} &=& \vroll{v|_p}\\
\vclos{\kappa}{\gamma}|_{\vclos{\kappa}{\rho}}&=&
\vclos{\kappa}{\gamma|_\rho}\\
{}[x_1 \mapsto v_1, \ldots,x_n \mapsto v_n]|_{[x_1 \mapsto p_1,
  \ldots,x_n \mapsto p_n]} &=& [x_1 := v_1|_{p_1},\ldots, x_n :=v_n|_{p_n}]
\end{eqnarray*}
For example, $(1,2) |_{(\vany,\vhole)} = (1,\vhole)$.

\begin{lemma}\label{lem:eqat-properties}
  For any $v$ and $p \sqleq v$, we have $v \eqat{p} v|_p$.
\end{lemma}
\begin{lemma}
  The set of partial values of a given value $v$ is a lattice with
  least element $\hole$, greatest element $v$ and the least upper
  bound operation $\sqcup$ as defined in \figref{lub}. 
\end{lemma}
\begin{lemma}
  For each $p$, $ \eqat{p}$ is a partial equivalence relation.  Moreover,
  whenever $p \sqcup p'$ is defined, we have $(\eqat{p \sqcup p'}) =
  (\eqat{p}) \cap (\eqat{p'})$, and whenever $p \sqleq p'$ we have
  $(\eqat{p}) \supseteq (\eqat{p'})$.
 \end{lemma}
 \begin{proof}
   To show $\eqat{p}$ is a partial equivalence relation, we must show
   that it is symmetric and transitive (but not necessarily
   reflexive).  Symmetry follows by straightforward induction on
   derivations.  Transitivity is by induction on $p$.  The second part
   follows by induction on the (partial recursive) definition of
   $\sqcup$.  The third part follows from the second by the fact that
   $p \sqleq p'$ holds if and only if $p \sqcup p' = p'$.  Full
   details of the proof are in \appref{eqat-properties-proof}.
 \end{proof}
 \begin{lemma}\label{lem:eqat-and}
   If $v \eqat{p} v'$ then $p \sqleq v$ and $p
   \sqleq v'$.  Conversely, if $p \sqleq v$ then $v \eqat{p} v$.
 \end{lemma}
 \begin{proof}
   By induction on derivations.  By symmetry it suffices to show by induction that $v
   \eqat{p} v'$ implies $p \sqleq v$.   The second part is straightforward. 
 \end{proof}

% It is worth noting that $\eqpat{p}$ actually says something stronger
% than the conclusion of the above lemma: namely, it says that $v$ and
% $v'$ match or mismatch $p$ in ``the same way''.  For example, $(2,2)
% \eqpat{(3,3)} (4,4)$  holds, because both corresponding components of
% pairs differ from the pattern, but $(2,3) \eqpat{(3,3)} (3,4)$ does not
% hold, because different parts of the two values match or mismatch the
% pattern.  

\input{fig-eqat}
\input{fig-lub}
%\input{fig-eqpat}

We also consider partial traces, usually written $S$, which are trace
expressions where some subexpressions have been replaced with $\hole$:
\begin{eqnarray*}
  S &::=& \cdots \mid \tremp
\end{eqnarray*}
As with patterns, we write $S \sqsubseteq T$ to indicate that $T$
matches $S$, that is, $S$ can be made equal to $T$ by filling in some
holes.

As mentioned at the beginning of this section, for the purpose of
disclosure and obfuscation analysis, we will consider the ``traces''
to be triples $(\gamma,T,v)$ where $T$ is consistent with $\gamma$ and
$v$, that is, $\gamma,T \trrun v$.  We refer to such a triple as a
\emph{consistent triple}.  Furthermore, to analyze forms of provenance based
on annotation we will consider consistent annotated triples
$(\hat{\gamma},T,\hat{v})$ where $\hat{v} = \extract(T,\hat{\gamma})$.
We consider trace or provenance queries built out of partial values
and partial traces.  We will later also consider queries derived from
different forms of provenance, based on annotated triples.

\todo{Compare with Kwasnikowska/van den Bussche traces.}

\begin{definition}
  \begin{enumerate}
  \item Let $\phi(\gamma)$ be a predicate on input environments.  An
    \emph{input query} $\IN{\gamma.\phi(\gamma)}$ is defined as
    $\{(\gamma,T,v) \mid \gamma,T \trrun v \text{ and }
    \phi(\gamma)\}$.  (Here, $\IN$ binds
    \highlight{$x$ in  $\phi(x)$}.)  As a special case, we write $\IN_\rho$ for
    $\IN{\gamma.(\rho \sqsubseteq \gamma)}$.  
  \item Let $\phi(v)$ be a predicate on output values.  An
    \emph{output query} $\OUT{v.\phi(v)}$ is defined as $ \{(\gamma,T,v)
    \mid \gamma,T \trrun v \text{ and } \phi(v)\}$.  (Here, $\OUT$
    binds \highlight{$x$ in $\phi(x)$}.) As a special
    case, we write $\OUT_p$ for $ \OUT{v.(p \sqsubseteq v)}$.
  \end{enumerate}
% \item A \emph{trace query} $\TRACE_S$ is defined as $\TRACE_S =
%   \{(\gamma,T,v) \mid S \subseteq v\}$.
% \item 
%   Suppose $\phi$ is a binary predicate relating annotated environments
%   and annotated values.  A \emph{provenance query}
%   $\PROV_{\extract,\phi}$ is defined as $\PROV_{\extract,\phi} =
%   \{(\gamma,T,v) \mid \phi(F(T,\hat{\gamma}),\hat(\gamma))\}$.
\end{definition}


==> space-tricks.tex <==
%space left between floats.
\setlength{\floatsep}{4mm}
% space between last top float or first bottom float and the text.
\setlength{\textfloatsep}{5mm}
% space left on top and bottom of an in-text float.
\setlength{\intextsep}{0mm}
% space above caption
\setlength{\abovecaptionskip}{0mm}
%space below caption
\setlength{\belowcaptionskip}{0mm}

%% Change figure handling
\renewcommand{\topfraction}{0.999999}
\renewcommand{\textfraction}{0.00001}
\renewcommand{\floatpagefraction}{0.9999999}


==> toplevel.tex <==
\section{Thoughts about toplevel language}

\newcommand{\PB}[1]{\llparenthesis #1 \rrparenthesis}
\newcommand{\extrace}[1]{\mathtt{trace}(#1)}
\newcommand{\trtrace}[1]{\extrace{#1}}
\newcommand{\vtrace}[3]{\mathtt{trace}\langle #1, #2, #3\rangle}
\newcommand{\extrupd}[3]{#1\PB{#2:=#3}}
\newcommand{\trtrupd}[3]{\extrupd{#1}{#2}{#3}}
\newcommand{\extrvar}[2]{#1\PB{#2}}
\newcommand{\trtrvar}[2]{\extrvar{#1}{#2}}
\newcommand{\extrval}[1]{\mathtt{val}(#1)}
\newcommand{\trtrval}[1]{\extrval{#1}}
\newcommand{\extrreplay}[1]{\mathtt{replay}(#1)}
\newcommand{\trtrreplay}[1]{\extrreplay{#1}}

\newcommand{\exwhereprov}[1]{\mathtt{where}(#1)}
\newcommand{\exdepprov}[1]{\mathtt{dep}(#1)}
\newcommand{\exexprprov}[1]{\mathtt{expr}(#1)}
\newcommand{\trwhereprov}[1]{\exwhereprov{#1}}
\newcommand{\trdepprov}[1]{\exdepprov{#1}}
\newcommand{\trexprprov}[1]{\exexprprov{#1}}
\newcommand{\exslice}[2]{\mathtt{slice}(#1,#2)}
\newcommand{\trslice}[2]{\exslice{#1}{#2}}

\begin{eqnarray*}
  e &::=& \cdots \mid \extrace{e} \mid \extrval{e} \mid \extrvar{e}{x} \mid
  \extrupd{e}{x}{e'} \mid \extrreplay{e}
\\
&\mid& \exwhereprov{e} \mid \exdepprov{e} \mid \exexprprov{e}
\\
v &::=& \cdots \mid \vtrace{v}{T}{\gamma}
\end{eqnarray*}

\begin{smathpar}
  \inferrule*{
    \gamma,e \eval v,T
  }{
    \gamma,\extrace{e} \eval \vtrace{v}{T}{\gamma}, \trtrace{T}
  }
\and
\inferrule*{
  \gamma,e \eval \vtrace{v_0}{T_0}{\gamma_0},T
}{
  \gamma,\extrval{e} \eval v,\extrval{T}
}
\and
\inferrule*{
  \gamma,e_1 \eval \vtrace{v_0}{T_0}{\gamma_0} \\
  \gamma,e_2 \eval v',T_2
}{
  \gamma, \extrupd{e_1}{x}{e_2} \eval \vtrace{v}{T}{\gamma_0[x:=v']}, \trtrupd{T_1}{x}{T_2}
}
\and 
\inferrule*{
  \gamma,e \eval \vtrace{v_0}{T_0}{\gamma_0} ,T
}{
  \gamma, \extrvar{e}{x} \eval \gamma_0(x), \trtrvar{T}{x}
}
\and
\inferrule*{
  \gamma,e \eval \vtrace{v}{T_0}{\gamma_0}, T\\
  \gamma_0, T_0 \eval v', T_0'
}{
  \gamma, \extrreplay{e} \eval \vtrace{v'}{T_0'}{\gamma_0}, \trtrreplay{T}
}
\and
\inferrule*{
  \gamma,e \eval \vtrace{v}{T}{\gamma} \\
  |\hat{\gamma_0}| = \gamma_0\\
  \where(T,\hat{\gamma_0}) = \hat{v}
}{
  \gamma,\exwhereprov{e} \eval \hat{v},\trwhereprov{T}
}
\and
\inferrule*{
  \gamma,e \eval \vtrace{v}{T}{\gamma} \\
  |\hat{\gamma_0}| = \gamma_0\\
  \dep(T,\hat{\gamma_0}) = \hat{v}
}{
  \gamma,\exdepprov{e} \eval \hat{v},\trdepprov{T}
}
\and
\inferrule*{
\gamma,e_1 \eval \vtrace{v_0}{T_0}{\gamma_0},T_1
\\
\gamma,e_2 \eval p,T_2
\\
p,T_0 \bwdslice S,\rho
}{
  \gamma,\exslice{e_1}{e_2} \eval \vtrace{p}{S}{\rho},\trslice{T_1}{T_2}
}
\end{smathpar}

I think it is safe to nest traces using the above language.



I may also want to allow programs to contain annotations, then all
values might potentially be annotated values.  The annotations woudl
on;y be used for provenance propagation and ignored / discarded otherwise.


Note that the slicing operation takes a partial value and produces a
partial trace (that is, a trace whose environment and return types
become partial).  This will require allowing partial values (values
with holes) as source-level syntax.  Partial values might also be
constructed using annotations (i.e., you create a value with an
annotation in it, and then make  partial value from it by replacing the
annotated part with a hole).

